ezDPS: An Efficient and Zero-Knowledge Machine Learning Inference Pipeline

Machine Learning as a service (MLaaS) permits resource-limited clients to access powerful data analytics services ubiquitously. Despite its merits, MLaaS poses significant concerns regarding the integrity of delegated computation and the privacy of the server's model parameters. To address this issue, Zhang et al. (CCS'20) initiated the study of zero-knowledge Machine Learning (zkML). Few zkML schemes have been proposed afterward; however, they focus on sole ML classification algorithms that may not offer satisfactory accuracy or require large-scale training data and model parameters, which may not be desirable for some applications. We propose ezDPS, a new efficient and zero-knowledge ML inference scheme. Unlike prior works, ezDPS is a zkML pipeline in which the data is processed in multiple stages for high accuracy. Each stage of ezDPS is harnessed with an established ML algorithm that is shown to be effective in various applications, including Discrete Wavelet Transformation, Principal Components Analysis, and Support Vector Machine. We design new gadgets to prove ML operations effectively. We fully implemented ezDPS and assessed its performance on real datasets. Experimental results showed that ezDPS achieves one-to-three orders of magnitude more efficient than the generic circuit-based approach in all metrics while maintaining more desirable accuracy than single ML classification approaches.

==> MLinstance.tex <==
\section{A Complete Machine Inference Pipeline}

\label{ml framework and circuits}
This section provides several specific examples as instances of the general machine learning algorithms. In each instantiated operator, the prover and the verifier would establish the circuit, public input, and witnesses using the gadgets and functions subprotocols above, then invoke the backend zero knowledge proof scheme to validate the integrity of the computation. We use $\mathrm{VC}(\mathrm{MLOP}, input, para)$ to represent the procedure of verifying computations without zero knowledge properties for operator Type-1, where $\mathrm{MLOP}$ is Machine Learning Operation. On the other hand, we adopt the notation $\mathrm{VC}_{zk}(\mathrm{MLOP}, input, para)$ to illustrate the verification that requires zero knowledge such as operator Type-2. Furthermore, instead of transforming the machine learning algorithms directly to circuits, we also propose multiple optimizations in this section, which significantly increase the efficiency. 


\subsection{Operator Type-1: Denoising}
\noindent For Operator Type-1, we instantiate it with discrete wavelet transformation (DWT). Specifically, we adopt the Daubechies DB4 wavelets algorithm. Normally speaking, the goal of DWT is denoising or extracting the features. In this paper, we mainly employ DWT to accomplish denoising. In order to do that, the DWT function exerts the wavelet coefficients on the raw data to project it to a new frequency domain space, and a thresholding function is operated to eliminate the high-frequency ingredient. In all, the DWT algorithm is composed of three parts: decomposition, thresholding, and reconstruction. The algorithms are described in Algorithm \ref{db decom}, \ref{db thre}, and \ref{db rec} in Appendix A.

\noindent Note that in DWT, the sever has no secret parameters. The goal in this stage is to verify the computation of the algorithms. The computation of DWT decomposition requires $8m$ constraints where $m$ is the number of features. In our paper, we transform the computation to the product of sums and reduce the number of constraints to constant. However, the transformation is not straightforward. Specifically, because the step length between two computations is two instead of one, there will be lots of extra intermediate values that have to be subtracted from the computation. To address this issue, we propose the splitting technique, which would first split the input vector and the kernels into two parts, respectively, and then performing the transformation. Formally, the initial decomposition stage is:

\begin{align}
	y_i &= \sum\limits_{j\in[1,4]}h_j\cdot x_{(2i+j-2)\mathsf{mod}m}, \qquad i\in\{1, m/2\}\\
	y_{\frac{m}{2}+i} &= \sum\limits_{j\in[1,4]}g_j\cdot x_{(2i+j-2)\mathsf{mod}m}, \qquad i\in\{1, m/2\}
\end{align}
where the vector $\myvec{y}=(y_1,y_2,…,y_m)$ is the result of the DWT decomposition. 

\noindent We can convert these equations to product of sums, such that

\begin{align}
	&(h_1+h_3)\cdot \sum\limits_{k=1}^{m/2}x_{2k-1}+(h_2+h_4)\cdot\sum\limits_{k=1}^{m/2}x_{2k}=\sum\limits_{i=1}^{m/2}y_i \\
	&(g_1+g_3)\cdot \sum\limits_{k=1}^{m/2}x_{2k-1}+(g_2+g_4)\cdot\sum\limits_{k=1}^{m/2}x_{2k}=\sum\limits_{i=m/2+1}^{m}y_i 
\end{align}

\noindent However, this simple representation is not sufficient to guarantee the relation because the prover cannot prove that each element of the output vector is valid, but only the sum is correct. To address this issue, the verifier could choose a random number $\alpha$ and send it to the prover. Then with the help of the powers of $\alpha$, the equations can be transformed to

\begin{align}
	(\alpha h_1+h_3)\cdot \sum\limits_{k=1}^{m/2}x_{2k-1}\alpha^{k-1}&+(\alpha h_2+h_4)\cdot \sum\limits_{k=1}^{m/2}x_{2k}\alpha^{k-1}\\ \nonumber
	&+(\alpha^{m/2}-1)h_3\cdot x_1+(\alpha^{m/2}-1)h_4\cdot x_2	=\sum\limits_{k=1}^{m/2}\alpha^ky_k\\
	(\alpha g_1+g_3)\cdot \sum\limits_{k=1}^{m/2}x_{2k-1}\alpha^{k-1}&+(\alpha g_2+g_4)\cdot \sum\limits_{k=1}^{m/2}x_{2k}\alpha^{k-1}\\ \nonumber
	&+(\alpha^{m/2}-1)g_3\cdot x_1+(\alpha^{m/2}-1)g_4\cdot x_2	=\sum\limits_{k=1}^{m/2}\alpha^ky_{k+m/2}
\end{align}

\noindent We provide an example of our split technique and illustrate it in Figure \ref{fig:dwt}. In all, via this transformation, the number of constraints is $16$ for each input vector $x$, which is much smaller than $8m$. The decomposition can be implemented by the Product of Sums gadget. 

\begin{figure}
	\centering
	\includegraphics[scale=0.5]{figures/dwt.png}
	\caption{DWT decomposition in product of sums.}
	\label{fig:dwt}
\end{figure}


\noindent The second part of DWT is the thresholding algorithm. We adopt the soft thresholding strategy in this step, such that
\begin{equation}
	y' = \left\{
	\begin{aligned}
		& sgn(y) (y - \lambda) &if |y| - \lambda > 0 \\
		& 0  &if |y| - \lambda < 0
	\end{aligned}
	\right.
\end{equation}
where $\lambda$ is the threshold, and $sgn(x)=1$ if $x>0$, otherwise $sgn(x)=-1$. The thresholding algorithm would check $y_i$ one by one for each $i$ in $[m/2+1,m]$. To convert the thresholding algorithm to R1CS relations, it suffices to employ the Comparison function. Other than the required binary representations of the elements that are engaged in the comparison, we also ask the Prover to provide $|y_i|$ and $sgn(y_i)$ as the auxiliary witnesses. With the help of the them, it is unneccessary to compare $y_i$ with zero for each $i$ in $[m/2+1, m]$. This would reduce the number of multiplication gates from $5n+14$ to $3n+9$ for each $y_i$, where $n$ is the length of the binary vectors. 

\noindent Finally, according to the algorithm, we have to reconstruct the data. DWT reconstruction is similar to the decomposition phase. Specifically, we transform the computation as

\begin{align}
	x'_{2k-1} &= \sum\limits_{j\in\{1,2\}}(Ih_{2j-1}\cdot y'_{(k+j-1)\mathsf{mod}\frac{m}{2}}+Ih_{2j}\cdot y'_{\frac{m}{2}+(k+j-1)\mathsf{mod}\frac{m}{2}}), \qquad k\in\{1, m/2\}\\
	x'_{2k} &= \sum\limits_{j\in\{1,2\}}(Ig_{2j-1}\cdot y'_{(k+j-1)\mathsf{mod}\frac{m}{2}}+Ig_{2j}\cdot y'_{\frac{m}{2}+(k+j-1)\mathsf{mod}\frac{m}{2}}), \qquad k\in\{1, m/2\}
\end{align}
where the vector $\myvec{y}'=(y_1,y_2,…,y_m)$ is the result of the thresholding stage, and $\myvec{x}'$ is the output of the reconstruction phase. The reconstruction can also be transformed as the product of sums with random numbers as the coefficients, such that

\begin{align}
	(\alpha Ih_1+Ih_3)\cdot \sum\limits_{k=1}^{m/2}y'_{k}\alpha^{k-1}&+(\alpha Ih_2+Ih_4)\cdot \sum\limits_{k=1}^{m/2}y'_{\frac{m}{2}+k}\alpha^{k-1}\\ \nonumber
	&+(\alpha^{m/2}-1)Ih_3\cdot y'_1+(\alpha^{m/2}-1)Ih_4\cdot y_{\frac{m}{2}+1}	=\sum\limits_{k=1}^{m/2}\alpha^k x'_{(2k+1)\mathsf{mod}m}\\
	(\alpha Ig_1+Ig_3)\cdot \sum\limits_{k=1}^{m/2}y'_{k}\alpha^{k-1}&+(\alpha Ig_2+Ig_4)\cdot \sum\limits_{k=1}^{m/2}y'_{\frac{m}{2}+k}\alpha^{k-1}\\ \nonumber
	&+(\alpha^{m/2}-1)Ig_3\cdot y'_1+(\alpha^{m/2}-1)Ig_4\cdot y_{\frac{m}{2}+1}	=\sum\limits_{k=1}^{m/2}\alpha^k x'_{(2k+2)\mathsf{mod}m}
\end{align}

\noindent In all, we present the verifying computation protocol for discrete wavelet denoising as follow.

\noindent\fbox{%
	\parbox{0.98\textwidth}{
		$(\{0,1\}, \myvec{O}_{dwt}) \leftarrow \mathrm{VC}(\mathrm{DWT}, \myvec{x}, \myvec{para}=(\myvec{h}, \myvec{g}, \myvec{Ih}. \myvec{Ig}, \lambda))$:
		\begin{align*}
			&(\mathcal{C}_0, \mathtt{PI}_0) \leftarrow \mathcal{G}_{\mathrm{PoSums}}(4)\\
			&\begin{aligned}
				&\witness{w}_0\leftarrow \text{The prover generates the witnesses for } \mathcal{C}_0 \text{ with corresponding inputs }\\
				&  \text{according to equation (9) and (10).}\\
			\end{aligned}\\
			&\text{For i in } [m/2+1, m]: (\text{Let k be the temporary index begin from 1})\\
			&\qquad(\mathcal{C}_k, \mathtt{PI}_k,\witness{w}_k) \leftarrow \mathcal{F}_{\mathrm{absolute}}(y_i, n) \\
			&\qquad(\mathcal{C}_{k+m/2}, \mathtt{PI}_{k+m/2}, \witness{w}_{k+m/2}) \leftarrow \mathcal{F}_{\mathrm{comparison}}((\witness{w}_k.abs, n, \lambda), n) \\ 
			&\qquad(\mathcal{C}_{m+2}, \mathtt{PI}_{m+2})\leftarrow \mathsf{R1CS}(sta_{dt})\\
			&\qquad \text{The prover generates all the witnesses for } \mathcal{C}_{m+2} \text{ with corresponding inputs}.\\
			&\begin{aligned}
				&\witness{w}_{m+3}\leftarrow \text{The prover generates the witnesses for } \mathcal{C}_0 \text{ with corresponding inputs }\\
				&  \text{according to equation (14) and (15).}\\
			\end{aligned}\\
			&(\mathcal{C}, \mathtt{PI}, \witness{w})\leftarrow  (\unionnew{\mathcal{C}_i},  \unionnew{0}{m+2}{\mathtt{PI}_i}, \unionnew{0}{m+3}{\witness{w}_i})\\
			&\{0, 1\}\leftarrow \mathrm{ZKP.B}(\mathcal{C}, \mathtt{PI}, \witness{w})\\
			&return (\{0, 1\}, \myvec{O}_{dwt})
		\end{align*}
}}

\subsection{Operator Type-2: Feature Extraction}
For Operator Type-2, we provide two instances for different goals. As an essential part of the general machine learning frameworks, feature extraction is practiced in various applications. Concretely, in this paper, we adopt the Principal Components Analysis (PCA) to extract the characteristics of the raw data and reduce its dimension. Suppose the raw data is of $m$ dimension. After being processed by PCA, the data dimension is reduced to $k$, $k < m$. The output of the PCA algorithm is called the principal component of the raw data. In this paper, we assume that the server holds a well-trained machine learning framework. Thus we only focus on the inference phase of PCA. The PCA inference algorithm is demonstrated in Algorithm \ref{pca} in Appendix A.

\noindent According to the PCA inference algorithm, we can change the representation into a product of sums to reduce the number of operations. In this step, both the input $x$ and the matrix $U$ are secrets. The relation can be transformed to product of sums by making use of the powers of a random number, such that
\begin{equation}
	\begin{aligned}
		&(u_{00}+\alpha u_{10}+...+\alpha^{k-1} u_{(k-1)0}) \cdot x_0 + (u_{01}+\alpha u_{11}+...+\alpha^{k-1} u_{(k-1)1} )\cdot x_1+...\\
		&+(u_{0(m-1)}+\alpha u_{1(m-1)}+...+\alpha^{(k-1)} u_{(k-1)(m-1)} )\cdot x_{m-1}\\
		&=o_0 + \alpha o_1+...+\alpha^{k-1} o_{k-1}
	\end{aligned}
\end{equation}
where $\alpha$ is a random number chosen by the client (verifier). Furthermore, to reduce the workload of the Prover, we can use the PRF function $PRF(\cdot)$ here to replace the exponential computation of $\alpha$. By using the product of sums, the number of constraints is reduced from $O(mk)$ to $O(m)$. Using this transformation above, we could implement the circuit of PCA by the Product of Sums gadget. 

\noindent\fbox{%
	\parbox{0.98\textwidth}{
		$(\{0, 1\}, \bm{O}_{pca}) \leftarrow \mathrm{VC}_{zk}(\mathrm{PCA}, \myvec{x}, \myvec{para}=PCA.\myvec{para})$:
		\begin{align*}
			&\text{The Verifier chooses a random seed } \alpha \text{and sends it to the Prover.}\\
			&\text{Both parties computes } \myvec{\alpha}=PRF(\alpha) \\
			&(\mathcal{C}_0, \mathtt{PI}_0) \leftarrow \mathcal{G}_{\mathrm{PoSums}}(k)\\
			&(\mathcal{C}_1, \mathtt{PI}_1) \leftarrow \mathcal{G}_{\mathrm{PoSums}}(m)\\
			&\witness{w}\leftarrow \text{The Prover computes the witnesses for } \mathcal{C}_0 \text{ and } \mathcal{C}_1 \text{ according to Algorithm } \ref{pca}.\\
			&(\mathcal{C}, \mathtt{PI})\leftarrow  (\unionnew{0}{1}{\mathcal{C}_i},  \unionnew{0}{1}{\mathtt{PI}_i})\\
			&\{0, 1\}\leftarrow \mathrm{ZKP.B}(\mathcal{C}, \mathtt{PI}, \witness{w})\\
			&return (\{0, 1\}, \bm{O}_{pca})
		\end{align*}
}}


\subsection{Operator Type-2: Inference}
The last component of our machine learning framework can also be viewed as an instance of the Operator Type-2. We instantiate the inference algorithm with Support Vector Machine (SVM), one of the most commonly used machine learning algorithms. It has satisfying performance for both classification (SVC) and regression (SVR), with solid mathematical principal supports. Similar to the previous sections, we only care about the inference phase of SVM. Note that SVM can be exerted on multiple types of datasets. The algorithm is described in Algorithm \ref{svm} in Appendix A. In order to make our instance more general, we adopt the kernel projection function to deal with the non-linear dataset and adopts the radial basis function (RBF) as an instance of the projection function illustrated in Section \ref{sec:function}. We give the subprotocol of the instantiated projection function below. 

\noindent\fbox{%
	\parbox{0.98\textwidth}{
		$(\mathcal{C}, \mathtt{PI}, \witness{w}) \leftarrow \mathcal{F}_{\mathrm{rbf}}((\myvec{x}, \myvec{x}_{sup}, \lambda), n)$:
		\begin{align*}
			&(\mathcal{C}_0, \mathtt{PI}_1) \leftarrow \mathsf{R1CS}(\{\mathcal{K}=-\lambda\Sigma(x_i-x_{sup_i})^2\})\\
			&\witness{w}_0\leftarrow \text{The prover generates all the witnesses for } \mathcal{C}_0 \text{ with correlonding inputs}.\\
			&(\mathcal{C}_1, \mathtt{PI}_1) \leftarrow \mathcal{G}_{\mathrm{Exp}}(n-1)\\
			&\witness{w}_1\leftarrow\text{The prover generates all the witnesses for } \mathcal{C}_1 \text{ with correlonding inputs}.\\
			&(\mathcal{C}, \mathtt{PI}, \witness{w})\leftarrow (\unionnew{0}{1}{\mathcal{C}_i},  \unionnew{0}{1}{\mathtt{PI}_i}, \unionnew{0}{1}{\witness{w}_i})\\
			&return (\mathcal{C}, \mathtt{PI}, \witness{w})
		\end{align*}
}}

\noindent where $\myvec{x}_{sup}$ is the support vector that is generated in the training procedure, and $\lambda$ is also the trainable parameter in the kernel projection function.

\noindent Moreover, we also expand the SVC from binary classification to multiple classification tasks and employ the One v.s. Rest strategy to accomplish it. Suppose there are $t$ classes in the dataset, then the well-trained inference model contains $t$ SVM models that in each model, one of the $t$ classes is designated as positive, and other classes are viewed as negative. The final prediction result would be the class with the highest decision function value. Specifically, the prediction can be represented as
\begin{equation}
	f_i(x) = \Sigma_j \beta_{ij}\mathcal{K}(\myvec{x}, \myvec{x}_{sup_{ij}}) + b_i
\end{equation}
where $i \in [0, t-1]$, $\beta_{ij}$ is the $j$th coefficient in the $i$th model, $\myvec{x}_{sup_{ij}}$ is the $j$th support vector in the $i$th model, and $\mathcal{K}(x, y)$ is the kernel function defined as $\mathcal{K}(x, y)=exp(-\gamma \times ||\myvec{x}-\myvec{y}||_2)$. To construct the circuit of the svm inference, it suffices to combine the kernel projection function, exponential function and absolute function together. As discussed before, the maximum function can be applied here to deal with the OvR strategy. Note that in this part, the use of the maximum function and the exponential gadgets in the RBF kernel projection function significantly decrease the number of constraints in the zero knowledge proof protocol.

\noindent\fbox{%
	\parbox{0.98\textwidth}{
		$(\{0, 1\}, \gamma) \leftarrow \mathrm{VC}_{zk}(\mathrm{SVM}, \myvec{x}, \myvec{para})$:
		\begin{align*}
			&\text{The Prover runs Algorithm } \ref{svm}: (\text{class } \gamma) \leftarrow SMV(\myvec{x}, \myvec{para}) \\
			&(\mathcal{C}_0, \mathtt{PI}_0) \leftarrow \mathsf{R1CS}(\{\Sigma_i a_i\times s_i+t=f\})\\
			&\text{For each support vector machine } f_i(\cdot):\\
			&\qquad \text{For each support vector } \myvec{sv}_{ij} \text{ in } \myvec{sv}_i:\\
			&\qquad \qquad (\mathcal{C}_{ij}, \mathtt{PI}_{ij}, \witness{w}_{ij}) \leftarrow \mathcal{F}_{\mathrm{rbf}}((\myvec{x}, \myvec{sv}_{ij}, \lambda), n)\\
			&\qquad \qquad \witness{w}_0 \leftarrow \text{The prover generates the witnesses for } \mathcal{C}_0 \text{ in each round according to Algorithm \ref{svm}}.\\
			&(\mathcal{C}_1, \mathtt{PI}_1, \witness{w}_1) \leftarrow \mathcal{F}_{\mathrm{maximum}}((f_\gamma(\myvec{x}), \bm{f}_{i\neq\gamma}(\myvec{x}), (m, n)))\\
			&(\mathcal{C}, \mathtt{PI}, \witness{w})\leftarrow  (\unionnew{}{}{\mathcal{C}},  \unionnew{}{}{\mathtt{PI}}, \union{}{}{\witness{w}})\\ 
			&\{0, 1\}\leftarrow \mathrm{ZKP.B}(\mathcal{C}, \mathtt{PI}, \witness{w})\\
			&return (\{0, 1\}, \gamma)
		\end{align*}
}}

\noindent In this section, we provide the verification for the instantiated operators separately, where both parties have to invoke the back-end zero knowledge proof scheme multiple times. However, it is also viable to combine several instantiated operators and invoke Protocol 1 only once. The modification needed is that at the end of each subprotocol of the algorithm, the prover and the verifier no longer call $\mathrm{ZKP.B}$ but return $(\mathcal{C}, \mathtt{PI}, \witness{w})$ directly. Both parties wait for the results of all subprotocols, and concatenate $\mathcal{C}, \mathtt{PI}, \witness{w}$ respectively. In the end, the prover and the verifier could use Protocol 1 for the final proof. 


\subsection{Putting Everything Together}
This section combines everything together and presents our zero knowledge proof protocol for the instantiated machine learning framework. Note that the circuits of the framework can be fully implemented by the gadgets and functions proposed in Section \ref{gadgets and functions}. We present our scheme in Protocol 2.

\noindent\fbox{%
	\parbox{0.98\textwidth}{
		Protocol 2 - (Zero Knowledge ML Framework (zkML)). Let $\lambda$ be the security parameter,  $\mathbb{F}$ be a prime field, ML be an instantiated machine learning framework with three components $(M_1, M_2, M_3)$, where $M_1$ is an instance of Operator Type-1, and $M_2$, $M_3$ are instances of Operator Type-2. Let $\mathcal{P}$ and $\mathcal{V}$ be the prover and verifier in the protocol respectively. The input of the Verifier is the vector $\myvec{x}$. 
		\begin{itemize}
			\item $(\{0,1\}, \myvec{O}_{dwt})\leftarrow \mathrm{VC}(\mathrm{DWT}, \myvec{x}, \mathrm{DWT}.\myvec{para})$
			\item $(\{0,1\}, \myvec{O}_{pca})\leftarrow \mathrm{VC}_{zk}(\mathrm{PCA}, \myvec{O}_{dwt}, \mathrm{PCA}.\myvec{para})$
			\item $(\{0,1\}, \gamma)\leftarrow \mathrm{VC}_{zk}(\mathrm{SVM}, \myvec{O}_{pca}, \mathrm{SVM}.\myvec{para})$
			\item If all checks pass, then $\mathcal{V}$ outputs $1$ and accept the classification result $\gamma$. Otherwise the Verifier will reject and abort.
		\end{itemize}
}}

\noindent \textbf{Complexity}. We adopt the zero knowledge proof scheme that is established on the R1CS relation as our backend. Therefore, the complexity of our scheme depends on the number of constraints in the complete machine learning pipeline. Suppose the dimension of the input vector is $m$, the dimension of PCA's output is $k$. Furthermore, there are $s$ classifying models in the support vector machine,  and there are in total $t$ support vectors that are trained and saved for all classes. The size of the R1CS relation would be $(3n+9)/2\times m +16$ for denoising, $m$ for feature reduction and $O(nt+kt+ns)$ for classification. Here $n$ is the dimension of the binary vectors for all the scalars in the field.

\noindent \textbf{Security}. We analyze the security of the instantiated zero-knowledge machine learning framework scheme. We have the following theorem.
\begin{theorem}
	\label{th:MLsecurity}
	Protocol 2 is a zero knowledge machine learning framework scheme as defined in definition 5.
\end{theorem}

\noindent \textit{Proof Sketch}. The proof of theorem \ref{th:MLsecurity} derives from the backend zero knowledge proof scheme adopted in Protocol 1. We provide the specific ways to construct the circuits and optimized them to reduce the number of constraints. These operations will not harm the security of the backend zero knowledge proof scheme.


==> reference.tex <==
\section*{Reference}

